G-Net: A Deep Learning Approach to G-computation for Counterfactual Outcome Prediction Under Dynamic Treatment Regimes

Counterfactual prediction is a fundamental task in decision-making. G-computation is a method for estimating expected counterfactual outcomes under dynamic time-varying treatment strategies. Existing G-computation implementations have mostly employed classical regression models with limited capacity to capture complex temporal and nonlinear dependence structures. This paper introduces G-Net, a novel sequential deep learning framework for G-computation that can handle complex time series data while imposing minimal modeling assumptions and provide estimates of individual or population-level time varying treatment effects. We evaluate alternative G-Net implementations using realistically complex temporal simulated data obtained from CVSim, a mechanistic model of the cardiovascular system.

==> tex/mimic.tex <==

%  In some critically ill patients, physicians administer fluid resuscitation to restore cardiac output and systemic blood pressure [4]. However, excessive fluid administration can cause fluid overload, a serious condition that can lead to complications such as pulmonary edema, heart failure, slow wound healing, or tissue degeneration [4]. Thus, control of fluid volume can be crucial to the survival of critically ill patients. When deciding on a fluid administration strategy, it can be difficult for physicians to weigh risks and benefits. Estimates of the probability of fluid overload under various fluid resuscitation strategies would be a great aid to decision-making. 
 
%  Realistic resuscitation strategies tend to be dynamic and time-varying, responding to changes in patients' hemodynamic status and possibly signs of overload. Further, there is treatment-confounder feedback where treatment (i.e. amount of fluid administered) at a given time influences confounders (e.g. blood pressure) at the following time, which in turn influence future treatment decisions. Hence, counterfactual prediction of fluid overload under alternative fluid resuscitation strategies calls for g-computation. We apply the G-net.% to estimate probability of fluid overload under alternative dynamic fluid administration strategies in ICU patients.  The intervention, the amount of fluid administered per hour, affects the health variables at the next timestep, and the health variables at the next timestep influence a physicians decision in fluid administration.

We also apply the G-Net to real ICU data from the MIMIC-3 dataset to make counterfactual predictions under alternative fluid administration strategies. In this section we will describe our dataset preparation process, experimental setup for this MIMIC dataset, and present our results on the MIMIC dataset. 
\subsection{Dataset Preparation}
%For our clinical problem of predicting fluid overload we prepare two datasets: the MIMIC-3 dataset and the CVSIM dataset.

\subsubsection{Data source}

Data were obtained from the Medical Information Mart for Intensive Care III (MIMIC-III) database available from PhysioNet \cite{MIMIC3,GoldbergerPhysioNet2000}. MIMIC III is a publicly available database which includes high resolution physiological data of over 38,000 distinct adult patients admitted to Beth Israel Deaconess Medical Center, Boston, MA, USA between 2001 – 2012 [27]. 
%There was an enterprise wide migration from CareVue Electronic Medical Record to Metavision (iMDsoft, Tel Aviv, Israel) in 2008, so for the sake of consistency, our analysis was restricted to patients admitted between 2008-2012.
\subsubsection{Cohort selection}
Our cohort comprises all 11,919 patients with documented fluid administration prior to ICU admission. Patients without pre-ICU fluid were excluded because total administered fluid volume is an important confounder, and a recorded pre-ICU fluid volume equal to 0 typically indicates missingness. The followup period was the earlier of 100 hours after admission to the ICU or the occurrence of an outcome or censoring event.
\subsubsection{Main outcome of interest}
%Unfortunately, there is no strict clinical definition of fluid overload available in our data. However, physicians usually put patients with too much fluid retention on diuretics. This is the primary use of diuretics in the ICU (except when patients are on mechanical ventilation). Thus, 
We use administration of diuretics as a proxy outcome for fluid overload. We say that a patient has become fluid overloaded the hour that physicians start administering diuretics for that patient. In our cohort, there are a total of 1,512 patients who experience fluid overload at some point during followup under our outcome definition. 
\subsubsection{Other stopping events, censoring events, and competing risks}
%Patients on mechanical ventilation are often given diuretics for reasons unrelated to fluid overload.
%we censor patients if they initiate mechanical ventilation (because we have no good outcome proxy for patients on mechanical ventilation).
When mechanical ventilation (MV) is initiated before a patient is put on diuretics, the usage of diuretics can no longer be used as an indication of fluid overload because diuretics may be prescribed for other reasons in this context. For this reason, we censor patients once they initiate MV. 

Death is a competing risk in that it precludes the possibility of future fluid overload and is itself an important outcome. Similarly, we assume that release from the ICU prior to the end of our followup period precludes fluid overload for the remainder of the followup period. In our cohort, 159 patients died before end of followup, 4922 were censored due to MV initiation, and 5310 were discharged from the ICU before end of followup.

\subsubsection{Time-varying treatment strategies}
We define the treatment at each hour to be the volume (in liters) of fluid administered in that hour.   
\subsubsection{Covariates}
Static (or baseline) covariates included race, age, height, service unit, and pre-existing comorbidities. (Static covariates are not themselves modeled by the G-net, but are predictors in regression models for outcomes and time-varying covariates.) Time-varying covariates, which change throughout a patient's stay, include vital signs and lab values.%Within the category of time-varying variables there are some that are categorical and some that are continuous, which are handled separately by our model through naive arbitrary ordering. Examples of categorical variables include mechanical ventilation as a binary indicator, vasopressor administration as a binary indicator, and death as a binary indicator. 
The full list of static and time-varying covariates is in Appendix A. 

\subsubsection{Data Binning and Processing}
Patient data was binned on an hourly basis. If multiple measurements of a covariate were made in the same hour, we took the average. If a measurement within an hour followed an outcome or censoring event, it was excluded. If a covariate measurement followed a treatment action (i.e. an alteration to the fluid volume rate), it was shifted to the following time bin to avoid improperly adjusting for post-treatment covariates.

The value of a time varying covariate at a given time was its most recent measured value, as this is the quantity observable to physicians that can influence treatment decisions and therefore must be adjusted for as a confounder. We also included variables indicating when each variable was last measured.  Initial values of covariates before they are first measured are set to zero.

\subsection{Experiments and Results}

For this application, we employed the simplest G-Net comprising two distinct LSTMs without a shared representation layer, one LSTM for categorical variables (vasopressor initiation, MV initiation, death, release from ICU, and fluid overload) and one for continuous variables (heart rate, mean arterial pressure, etc.). This is the model described in Section 4 and illustrated in figure BLANK. Because the simplest model performed well on predictive checks (described below), we deemed it unnecessary to employ more complex models such as the attention model that was required for stable performance in the CVSim data. [[TODO: PROVIDE SOME JUSTIFICATION OF WHY WE DID NOT USE ATTN MODEL]]

The MIMIC-3 dataset only contains data generated under the observational regime, so we cannot directly evaluate counterfactual predictions produced by the G-Net. Instead, we take Cain et al.'s approach to evaluation in which we perform sanity checks on the ``factual'' predictive performance of the G-Net. That is, we use the G-net to simulate data under the observational regime (or ``natural course'') and perform predictive checks comparing the distribution of simulated data to the actually observed data. 

To estimate outcomes under the observational regime, we simply input an estimate of the (stochastic) observed treatment strategy where we would ordinarily input a counterfactual treatment strategy of interest in the g-computation algorithm. The predictive check works as follows: We first fit our G-net on the training set to have it learn to predict both the covariates ($L$) and the treatments ($A$) at each time step. Using our G-net, we simulate each patient forward $w$ time steps from baseline under the stochastic treatment strategy defined by our predictive model for treatment, stopping as necessary based on previously discussed stopping events. We then compare survival curves in the simulated and real data for each of the stopping events.

Figures 8 and 9 show the results of this predictive check. Figure 8 contains all the survival curves for the outcome and stopping events. Figure 9 show the population average of the G-Net predictions against the acutal population averages of a few covariates over the simulation window. 
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_diuretic_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_death_2_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_release_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_mv_test.png}
    \caption{Survival Curves for Outcome of Interest(diuretics initiation) and censoring events(death, release, mv initiation)}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_resprate_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_diasbp_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_sysbp_test.png}
    \includegraphics[width=0.75\linewidth]{MIMIC/survival_curve_YasL0_urineoutput_test.png}
    \caption{Population Average Trajectory Plots For a few Covariates of Interest. Please note that the y-axis is the original, clinically interpret-able ranges for these values, not the normalized ranges. For full results, please see the Appendix.}
    \label{fig:my_label}
\end{figure}

Reassured that our G-net appears to perform well at the task of prediction under the natural course, we can trust its counterfactual predictions to the extent that unverifiable Assumptions 1 and 2 hold.

%Since we do not have the data for a counterfactual regime for the MIMIC dataset and only data from the observational regime, we can only perform a sanity check on the predictive abilities of our model on the MIMIC-3 Dataset. The predictive check would work as follows: We first fit our G-net on the training set to have it learn to predict both the covariates($L$) and the treatments($A$) at each timestep. Using our G-net, we simulate patient trajectories forward, $w$ timesteps, censoring as necessary, based on our previously discussed censoring criteria.  For each patient we simulate forward 500 trajectories. If a trajectory is censored in less than $w$ timesteps, the censoring variables are padded with their final values until $w$; other covariates are padded with NANs. We then take the average value of each covariate and the outcome at each timestep $t$ (where $t = 1:w$) across all patient's trajectories, resulting in a time-to-event curve for each variable, where the x-axis is the time axis and the y-axis is the variable value. The observed trajectories' survival curves are also plotted alongside the predicted trajectories' survival curves for a visual comparison of the distributions of the predicted trajectories and the observed trajectories from the MIMIC dataset. These results are presented in Section 8.1. 

In figure 10, we display counterfactual predictions for a few real patients under aggressive and conservative fluid strategies. Under the aggressive counterfactual strategy, we administer 1 L of fluid if mean blood pressure is below 65. Under the passive counterfactual strategy, we administer 0.2 L of fluid if mean blood pressure is below 55. [[TODO: I WILL UPLOAD PLOTS FOR CF STRATEGIES TOMORROW (RUI)]]
